3D Morphology of Open Clusters in the Solar Neighborhood with Gaia EDR3 II: Hierarchical Star Formation Revealed by Spatial and Kinematic Substructures

We identify members of 65 open clusters in the solar neighborhood using the machine-learning algorithm StarGO based on Gaia EDR3 data. After adding members of twenty clusters from previous studies (Pang et al. 2021a,b; Li et al. 2021) we obtain 85 clusters, and study their morphology and kinematics. We classify the substructures outside the tidal radius into four categories: filamentary (f1) and fractal (f2) for clusters $<100$ Myr, and halo (h) and tidal-tail (t) for clusters $>100$ Myr. The kinematical substructures of f1-type clusters are elongated; these resemble the disrupted cluster Group X. Kinematic tails are distinct in t-type clusters, especially Pleiades. We identify 29 hierarchical groups in four young regions (Alessi 20, IC 348, LP 2373, LP 2442); ten among these are new. The hierarchical groups form filament networks. Two regions (Alessi 20, LP 2373) exhibit global "orthogonal" expansion (stellar motion perpendicular to the filament), which might cause complete dispersal. Infalling-like flows (stellar motion along the filament) are found in UBC 31 and related hierarchical groups in the IC 348 region. Stellar groups in the LP 2442 region (LP 2442 gp 1-5) are spatially well-mixed but kinematically coherent. A merging process might be ongoing in the LP 2442 subgroups. For younger systems ($\lesssim30$ Myr), the mean axis ratio, cluster mass and half-mass radius tend to increase with age values. These correlations between structural parameters may imply two dynamical processes occurring in the hierarchical formation scenario in young stellar groups: (1) filament dissolution and (2) sub-group mergers.

==> Pang et al. 2022 3d OC/Parameters_85_overleaf_updated6.tex <==
\rm Alessi\,3	&	109.139147	&	-46.074168	&	277.3	&	1.22	&	-9.804	&	11.945	&	631	&	124.6	&	6.8	&	7.0	&	165	&	0.52	&	\rm t	\\
\rm Alessi\,5	&	160.927572	&	-61.087405	&	397.7	&	11.13	&	-15.354	&	2.535	&	52	&	244.0	&	4.4	&	8.7	&	279	&	0.89	&		\\
\rm Alessi\,9	&	265.946512	&	-47.070299	&	207.6	&	-6.59	&	10.036	&	-9.109	&	265	&	61.7	&	4.5	&	5.5	&	79	&	0.62	&		\\
\rm Alessi\,20	&	2.970330	&	58.532158	&	423.4	&	-5.74	&	7.904	&	-2.378	&	9	&	240.4	&	11.1	&	8.7	&	349	&	0.32	&	\rm f1	\\
\rm Alessi\,20\,gp1$^a$	&	356.035534	&	56.078582	&	411.9	&	-10.68	&	8.130	&	-3.347	&	12	&	173.2	&	13.6	&	7.8	&	265	&	0.18	&	\rm f2	\\
\rm Alessi\,20\,isl1$^a$	&	11.906507	&	50.262109	&	458.9	&	-3.21	&	7.391	&	-3.108	&	100	&	97.6	&	7.5	&	6.4	&	107	&	0.41	&		\\
\rm Alessi\,24	&	260.842675	&	-62.670437	&	484.2	&	12.10	&	-0.441	&	-8.948	&	88	&	119.1	&	4.6	&	6.9	&	138	&	0.73	&		\\
\rm Alessi\,62	&	284.025507	&	21.581477	&	618.9	&	12.77	&	0.256	&	-1.120	&	692	&	144.1	&	5.7	&	7.3	&	139	&	0.63	&		\\
\rm ASCC\,16	&	81.160907	&	1.558096	&	346.4	&	20.95	&	1.299	&	-0.013	&	11	&	241.7	&	6.0	&	8.7	&	373	&	0.74	&		\\
\rm ASCC\,19	&	82.011177	&	-1.975022	&	354.7	&	24.50	&	1.118	&	-1.173	&	9	&	198.5	&	7.8	&	8.2	&	323	&	0.53	&	\rm f2	\\
\rm ASCC\,58	&	153.712881	&	-55.126490	&	477.1	&	11.69	&	-13.353	&	2.703	&	52	&	254.9	&	9.9	&	8.9	&	328	&	0.44	&	\rm f2	\\
\rm ASCC\,105	&	295.444115	&	27.493132	&	557.8	&	-15.46	&	1.426	&	-1.602	&	74	&	67.5	&	5.9	&	5.7	&	67	&	0.48	&	\rm f1	\\
\rm ASCC\,127	&	346.610023	&	65.131092	&	374.4	&	-11.89	&	7.424	&	-1.785	&	15	&	183.0	&	11.9	&	7.9	&	260	&	0.29	&	\rm f1	\\
\rm BH\,99	&	159.413798	&	-59.062415	&	446.9	&	13.08	&	-14.470	&	1.089	&	81	&	556.7	&	8.3	&	11.5	&	730	&	0.63	&	\rm f2	\\
\rm BH\,164	&	222.290304	&	-66.446488	&	419.8	&	-0.03	&	-7.404	&	-10.689	&	65	&	194.5	&	5.3	&	8.1	&	243	&	0.72	&		\\
\rm Blanco\,1$^b$	&	1.536331	&	-29.975190	&	236.4	&	6.21	&	18.708	&	2.606	&	100	&	342.9	&	6.7	&	10.2	&	703	&	0.64	&	\rm t	\\
\rm Collinder\,69	&	83.809113	&	9.809913	&	399.0	&	25.89	&	1.300	&	-2.113	&	14	&	401.8	&	8.1	&	10.3	&	620	&	0.63	&	\rm f1	\\
\rm Collinder\,135$^b$	&	109.553612	&	-37.079084	&	302.8	&	16.12	&	-10.101	&	6.165	&	40	&	253.2	&	9.7	&	8.9	&	377	&	0.41	&	\rm f2	\\
\rm Collinder\,140	&	110.944634	&	-32.063703	&	384.5	&	19.07	&	-8.073	&	4.769	&	50	&	179.6	&	10.2	&	7.9	&	241	&	0.42	&	\rm f2	\\
\rm Collinder\,350	&	267.003004	&	1.452913	&	367.8	&	-14.79	&	-4.933	&	-0.060	&	589	&	149.4	&	6.6	&	7.4	&	156	&	0.51	&	\rm t	\\
\rm Coma\,Berenices$^b$	&	186.034554	&	25.539697	&	85.6	&	0.04	&	-12.018	&	-8.940	&	700	&	101.6	&	4.7	&	6.8	&	158	&	0.59	&	\rm t	\\
\rm Group\,X	&	217.766195	&	54.432658	&	99.6	&	-6.50	&	-16.051	&	-2.802	&	400	&	99.5	&	14.5	&	6.8	&	187	&	0.11	&	d	\\
\rm Gulliver\,6	&	83.207952	&	-1.711134	&	413.3	&	30.27	&	0.128	&	-0.269	&	7	&	168.5	&	7.3	&	7.7	&	284	&	0.54	&	\rm f1	\\
\rm Gulliver\,21	&	106.889853	&	-25.471498	&	652.5	&	41.25	&	-1.875	&	4.226	&	275	&	83.3	&	4.9	&	6.1	&	74	&	0.68	&		\\
\rm Huluwa\,1$^b$	&	122.390262	&	-47.017897	&	354.7	&	17.00	&	-6.374	&	9.360	&	12	&	724.0	&	14.6	&	12.6	&	1294	&	0.39	&	\rm f1	\\
\rm Huluwa\,2$^b$	&	121.163632	&	-48.884799	&	398.8	&	20.65	&	-5.525	&	8.226	&	11	&	467.4	&	15.3	&	10.9	&	743	&	0.26	&	\rm f1	\\
\rm Huluwa\,3$^b$	&	117.397635	&	-46.600642	&	394.7	&	21.76	&	-4.706	&	8.960	&	11	&	372.8	&	7.9	&	10.1	&	588	&	0.66	&		\\
\rm Huluwa\,4$^b$	&	125.994565	&	-41.178685	&	341.8	&	19.83	&	-7.115	&	10.021	&	10	&	180.7	&	14.8	&	7.9	&	347	&	0.28	&	\rm f1	\\
\rm Huluwa\,5$^b$	&	126.933768	&	-34.930350	&	355.0	&	15.69	&	-7.007	&	10.779	&	8	&	60.8	&	4.7	&	5.5	&	102	&	0.65	&	\rm f1	\\
\rm IC\,348	&	56.093028	&	32.173637	&	316.5	&	16.99	&	4.415	&	-6.407	&	5	&	142.2	&	4.1	&	7.3	&	211	&	0.73	&		\\
\rm IC\,2391$^b$	&	130.229784	&	-52.990392	&	151.3	&	15.01	&	-24.641	&	23.309	&	50	&	140.2	&	2.5	&	7.6	&	219	&	0.99	&		\\
\rm IC\,2602$^b$	&	160.515429	&	-64.443674	&	151.4	&	16.57	&	-17.691	&	10.695	&	45	&	188.1	&	3.7	&	8.4	&	318	&	0.91	&		\\
\rm IC\,4665$^b$	&	266.568565	&	5.608075	&	347.4	&	-13.19	&	-0.845	&	-8.543	&	36	&	158.5	&	6.0	&	7.9	&	197	&	0.72	&		\\
\rm IC\,4756	&	279.617685	&	5.430164	&	473.7	&	-24.37	&	1.236	&	-4.991	&	955	&	508.0	&	8.2	&	11.2	&	497	&	0.70	&	\rm t	\\
\rm LP\,2371	&	82.056845	&	1.632299	&	367.0	&	29.36	&	-0.549	&	0.746	&	20	&	81.0	&	5.1	&	6.1	&	103	&	0.67	&		\\
\rm LP\,2373	&	83.844838	&	-5.670678	&	386.9	&	21.01	&	1.621	&	-1.097	&	9	&	98.0	&	7.9	&	6.5	&	153	&	0.39	&	\rm f1	\\
\rm LP\,2373\,gp1$^a$	&	81.170979	&	-2.515377	&	335.6	&	22.52	&	1.104	&	-0.277	&	11	&	187.4	&	12.0	&	8.0	&	341	&	0.23	&	\rm f1	\\
\rm LP\,2373\,gp2	&	81.836831	&	1.892265	&	349.3	&	17.77	&	1.543	&	-0.545	&	9	&	543.0	&	11.6	&	11.4	&	884	&	0.47	&	\rm f1	\\
\rm LP\,2373\,gp3	&	83.509434	&	-0.498267	&	349.1	&	20.10	&	1.671	&	-0.932	&	6	&	111.3	&	9.0	&	6.7	&	177	&	0.34	&	\rm f1	\\
\rm LP\,2373\,gp4	&	84.260923	&	-2.053777	&	363.0	&	20.67	&	1.708	&	-1.310	&	6	&	296.2	&	9.9	&	9.3	&	490	&	0.48	&	\rm f2	\\
\rm LP\,2383	&	95.335972	&	-16.218225	&	364.3	&	24.81	&	-5.420	&	5.068	&	50	&	280.7	&	12.8	&	9.2	&	475	&	0.34	&	\rm f2	\\
\rm LP\,2388	&	127.066134	&	-47.931643	&	497.3	&	24.94	&	-5.923	&	6.884	&	200	&	149.4	&	6.8	&	7.4	&	199	&	0.53	&		\\
\rm LP\,2428	&	43.296942	&	68.875038	&	436.1	&	-1.96	&	1.428	&	-7.976	&	200	&	111.0	&	6.0	&	6.7	&	142	&	0.58	&		\\
\rm LP\,2429	&	84.460533	&	57.169259	&	479.5	&	-6.36	&	-3.222	&	-3.992	&	1150	&	148.0	&	6.1	&	7.4	&	179	&	0.61	&	\rm t	\\
\rm LP\,2439	&	103.540197	&	-5.896183	&	283.9	&	23.13	&	-7.336	&	-2.457	&	25	&	143.0	&	6.5	&	7.3	&	243	&	0.54	&	\rm f2	\\
\rm LP\,2441	&	279.297560	&	-14.225387	&	280.4	&	-21.37	&	-1.772	&	-9.437	&	75	&	187.8	&	8.9	&	8.0	&	226	&	0.46	&	\rm f2	\\
\rm LP\,2442	&	250.101032	&	-39.560185	&	175.8	&	1.45	&	-11.929	&	-21.288	&	15	&	318.7	&	6.2	&	9.6	&	662	&	0.70	&	\rm f2	\\
\rm LP\,2442\,gp1$^a$	&	242.331352	&	-22.907537	&	138.9	&	-7.47	&	-11.731	&	-24.786	&	8	&	111.6	&	8.7	&	6.7	&	220	&	0.29	&	\rm f2	\\
\rm LP\,2442\,gp2$^a$	&	243.556287	&	-23.095881	&	141.1	&	-6.73	&	-8.884	&	-24.562	&	8	&	151.8	&	7.9	&	7.5	&	363	&	0.47	&	\rm f2	\\
\rm LP\,2442\,gp3$^a$	&	241.119806	&	-22.113086	&	143.4	&	-6.21	&	-12.199	&	-23.174	&	8	&	64.0	&	6.4	&	5.6	&	136	&	0.38	&	\rm f2	\\
\rm LP\,2442\,gp4$^a$	&	244.532627	&	-25.119324	&	153.7	&	-4.34	&	-10.774	&	-21.905	&	8	&	113.0	&	10.2	&	6.8	&	284	&	0.26	&	\rm f2	\\
\rm LP\,2442\,gp5$^a$	&	242.398266	&	-20.348396	&	153.9	&	-5.61	&	-9.609	&	-21.354	&	8	&	76.9	&	9.8	&	6.0	&	163	&	0.26	&	\rm f2	\\
\rm Mamajek\,4	&	276.232342	&	-51.301191	&	449.9	&	-28.90	&	4.413	&	-21.456	&	372	&	281.5	&	17.7	&	9.2	&	320	&	0.21	&	\rm t	\\
\rm NGC\,1901	&	79.555700	&	-68.181508	&	417.8	&	0.67	&	1.681	&	12.694	&	850	&	124.8	&	6.7	&	7.0	&	144	&	0.52	&		\\
\rm NGC\,1977	&	83.847140	&	-4.973568	&	392.3	&	25.28	&	1.120	&	-0.547	&	3	&	107.7	&	4.7	&	6.7	&	202	&	0.76	&		\\
\rm NGC\,1980	&	83.804049	&	-5.865419	&	383.6	&	23.50	&	1.119	&	0.344	&	6	&	753.2	&	7.6	&	12.7	&	1298	&	0.81	&		\\
\rm NGC\,2232$^b$	&	96.721725	&	-4.630480	&	320.0	&	26.37	&	-4.626	&	-1.851	&	25	&	205.8	&	6.8	&	8.6	&	281	&	0.57	&	\rm f1	\\
\rm NGC\,2422$^b$	&	114.122352	&	-14.484943	&	476.4	&	35.86	&	-7.051	&	1.026	&	73	&	480.2	&	4.9	&	11.4	&	466	&	0.90	&		\\
\rm NGC\,2451A$^b$	&	115.754528	&	-38.264155	&	192.6	&	22.62	&	-20.954	&	15.333	&	58	&	182.2	&	4.9	&	8.3	&	311	&	0.82	&		\\
\rm NGC\,2451B	&	116.079334	&	-38.016157	&	363.2	&	16.65	&	-9.575	&	4.846	&	50	&	276.1	&	8.0	&	9.1	&	400	&	0.54	&	\rm f2	\\
\rm NGC\,2516$^b$	&	119.492636	&	-60.786856	&	410.6	&	24.22	&	-4.620	&	11.203	&	123	&	1973.3	&	7.9	&	18.3	&	2690	&	0.88	&	\rm t	\\
\rm NGC\,2547$^b$	&	122.490342	&	-49.178877	&	387.2	&	13.42	&	-8.562	&	4.365	&	40	&	303.9	&	5.6	&	9.8	&	452	&	0.71	&	\rm f2	\\
\rm NGC\,3228	&	155.377537	&	-51.880903	&	482.2	&	16.49	&	-14.848	&	-0.573	&	63	&	84.4	&	6.3	&	6.1	&	81	&	0.50	&		\\
\rm NGC\,3532	&	166.388592	&	-58.701886	&	478.3	&	5.44	&	-10.400	&	5.235	&	398	&	2210.5	&	7.4	&	18.2	&	2559	&	0.90	&	\rm h	\\
\rm NGC\,6405	&	265.095354	&	-32.227742	&	457.6	&	-8.12	&	-1.383	&	-5.859	&	79	&	596.9	&	5.3	&	11.8	&	654	&	0.87	&		\\
\rm NGC\,6475	&	268.466733	&	-34.828885	&	279.5	&	-14.55	&	3.083	&	-5.403	&	186	&	1024.5	&	6.1	&	14.1	&	1157	&	0.86	&	\rm h	\\
\rm NGC\,6633$^b$	&	276.890553	&	6.680996	&	394.0	&	-28.11	&	1.242	&	-1.800	&	426	&	337.3	&	5.3	&	10.2	&	300	&	0.82	&		\\
\rm NGC\,6774$^b$	&	289.091567	&	-16.317354	&	306.4	&	42.24	&	-0.889	&	-26.656	&	2650	&	152.6	&	4.7	&	7.8	&	154	&	0.76	&		\\
\rm NGC\,7058	&	320.451323	&	50.821327	&	365.2	&	-19.21	&	7.483	&	2.772	&	80	&	126.8	&	3.4	&	7.0	&	190	&	0.83	&		\\
\rm NGC\,7092	&	322.782191	&	48.247177	&	297.1	&	-5.29	&	-7.387	&	-19.718	&	350	&	193.1	&	6.5	&	8.1	&	303	&	0.61	&	\rm t	\\
\rm Pleiades$^b$	&	56.637062	&	24.132371	&	135.9	&	5.72	&	19.945	&	-45.365	&	125	&	744.0	&	4.7	&	12.7	&	1407	&	0.86	&	\rm t	\\
\rm Praesepe	&	130.008023	&	19.601297	&	185.0	&	35.00	&	-35.904	&	-12.864	&	700	&	601.8	&	4.7	&	11.8	&	982	&	0.92	&	\rm h	\\
\rm Roslund\,5	&	302.659299	&	33.751082	&	540.5	&	-16.61	&	2.078	&	-1.183	&	98	&	191.5	&	6.8	&	8.1	&	207	&	0.57	&	\rm f2	\\
\rm RSG\,7	&	343.949646	&	59.772583	&	419.3	&	-8.55	&	4.760	&	-2.244	&	70	&	67.6	&	4.6	&	5.7	&	69	&	0.59	&		\\
\rm RSG\,8	&	345.689844	&	59.113059	&	474.6	&	-8.68	&	5.665	&	-1.663	&	18	&	342.8	&	22.0	&	9.8	&	408	&	0.09	&	\rm f2	\\
\rm Stephenson\,1	&	283.406739	&	36.720713	&	358.2	&	-19.13	&	1.075	&	-3.020	&	46	&	263.4	&	7.0	&	9.0	&	407	&	0.58	&	\rm f1	\\
\rm Stock\,1	&	294.146449	&	25.145437	&	406.3	&	-19.75	&	6.105	&	0.205	&	470	&	136.3	&	4.6	&	7.2	&	125	&	0.77	&		\\
\rm Stock\,12	&	353.914758	&	52.678590	&	437.7	&	-2.18	&	8.553	&	-1.920	&	112	&	122.0	&	4.3	&	6.9	&	124	&	0.73	&		\\
\rm Stock\,23	&	49.134918	&	60.355183	&	606.7	&	-18.57	&	-4.313	&	-1.010	&	94	&	106.0	&	9.1	&	6.6	&	78	&	0.37	&	\rm f1	\\
\rm UBC\,7$^b$	&	106.935171	&	-37.677240	&	278.3	&	16.78	&	-9.730	&	7.004	&	40	&	192.3	&	7.6	&	8.1	&	336	&	0.54	&	\rm f2	\\
\rm UBC\,19	&	56.443686	&	29.936422	&	399.7	&	19.45	&	2.825	&	-5.217	&	7	&	42.2	&	6.1	&	4.9	&	57	&	0.38	&		\\
\rm UBC\,31	&	60.707033	&	32.542298	&	365.0	&	20.89	&	3.698	&	-5.370	&	12	&	260.0	&	14.7	&	8.9	&	353	&	0.13	&	\rm f1	\\
\rm UBC\,31\,gp1$^a$	&	63.563584	&	32.027203	&	339.2	&	20.90	&	3.766	&	-5.937	&	12	&	58.9	&	10.7	&	5.4	&	80	&	0.13	&	\rm f1	\\
\rm UBC\,31\,gp2$^a$	&	57.959044	&	35.028000	&	381.4	&	23.12	&	3.385	&	-4.450	&	10	&	185.1	&	10.7	&	8.0	&	213	&	0.27	&	\rm f1	\\
\rm UPK\,82	&	298.265305	&	26.504003	&	542.2	&	-12.72	&	2.258	&	-2.117	&	81	&	57.6	&	4.8	&	5.4	&	61	&	0.56	&		\\


==> Pang et al. 2022 3d OC/table3_data.tex <==
\rm Alessi\,3	&	1.9	&	5.76	\pm	1.33	&	4.53	\pm	0.21	&	3.4	\pm	0.26	&	0.79	\pm	0.19	&	0.59	\pm	0.14	&	15.02	&	77.1	&	\rm III	\\
\rm Alessi\,5	&	2.7	&	5.29	\pm	2.87	&	4.85	\pm	0.38	&	3.17	\pm	0.46	&	0.92	\pm	0.5	&	0.6	\pm	0.34	&	12.49	&	17.37	&	\rm III	\\
\rm Alessi\,9	&	1.7	&	6.34	\pm	1.02	&	3.1	\pm	0.16	&	2.73	\pm	0.21	&	0.49	\pm	0.08	&	0.43	\pm	0.08	&	21.49	&	34.66	&	\rm II	\\
\rm Alessi\,20	&	3.0	&	6.35	\pm	3.47	&	4.52	\pm	0.44	&	3.73	\pm	0.51	&	0.71	\pm	0.39	&	0.59	\pm	0.33	&	22.25	&	30.53	&		\\
\rm Alessi\,20\,gp1$^a$	&	3.0	&	6.29	\pm	3.42	&	5.38	\pm	0.43	&	3.97	\pm	0.52	&	0.86	\pm	0.47	&	0.63	\pm	0.35	&	14.32	&	15.04	&	\rm III	\\
\rm Alessi\,20\,isl1$^a$	&	3.4	&	6.0	\pm	4.4	&	4.25	\pm	0.51	&	3.16	\pm	0.59	&	0.71	\pm	0.53	&	0.53	\pm	0.4	&	38.54	&	89.49	&		\\
\rm Alessi\,24	&	4.0	&	5.41	\pm	6.41	&	4.42	\pm	0.65	&	2.75	\pm	0.73	&	0.82	\pm	0.97	&	0.51	\pm	0.62	&	16.37	&	15.38	&	\rm I	\\
\rm Alessi\,62	&	3.8	&	6.86	\pm	5.48	&	4.08	\pm	0.59	&	3.16	\pm	0.65	&	0.59	\pm	0.48	&	0.46	\pm	0.38	&	7.29	&	40.47	&		\\
\rm ASCC\,16	&	2.4	&	6.41	\pm	2.13	&	4.93	\pm	0.31	&	3.81	\pm	0.36	&	0.77	\pm	0.26	&	0.59	\pm	0.21	&	22.25	&	62.74	&		\\
\rm ASCC\,19	&	2.6	&	6.95	\pm	2.65	&	5.11	\pm	0.36	&	4.03	\pm	0.42	&	0.74	\pm	0.28	&	0.58	\pm	0.23	&	16.61	&	3.24	&		\\
\rm ASCC\,58	&	4.0	&	6.42	\pm	6.11	&	5.42	\pm	0.63	&	4.32	\pm	0.69	&	0.84	\pm	0.81	&	0.67	\pm	0.65	&	13.64	&	33.7	&		\\
\rm ASCC\,105	&	3.2	&	4.56	\pm	4.06	&	3.97	\pm	0.5	&	2.75	\pm	0.57	&	0.87	\pm	0.78	&	0.6	\pm	0.55	&	16.22	&	34.89	&	\rm III	\\
\rm ASCC\,127	&	2.5	&	5.96	\pm	2.37	&	5.15	\pm	0.33	&	3.7	\pm	0.4	&	0.86	\pm	0.35	&	0.62	\pm	0.26	&	22.88	&	18.9	&	\rm III	\\
\rm BH\,99	&	3.8	&	7.69	\pm	5.64	&	5.83	\pm	0.61	&	4.77	\pm	0.67	&	0.76	\pm	0.56	&	0.62	\pm	0.46	&	11.51	&	13.79	&		\\
\rm BH\,164	&	3.6	&	6.97	\pm	5.01	&	5.26	\pm	0.56	&	2.78	\pm	0.63	&	0.75	\pm	0.55	&	0.4	\pm	0.3	&	3.82	&	65.19	&	\rm III	\\
\rm Collinder\,69	&	3.1	&	7.64	\pm	3.87	&	5.94	\pm	0.48	&	5.34	\pm	0.55	&	0.78	\pm	0.4	&	0.7	\pm	0.36	&	22.77	&	74.18	&		\\
\rm Collinder\,135$^b$	&	2.2	&	7.17	\pm	1.77	&	6.42	\pm	0.27	&	3.67	\pm	0.31	&	0.9	\pm	0.22	&	0.51	\pm	0.13	&	20.74	&	47.57	&	\rm I	\\
\rm Collinder\,140	&	2.8	&	6.64	\pm	3.09	&	5.9	\pm	0.42	&	3.29	\pm	0.46	&	0.89	\pm	0.42	&	0.5	\pm	0.24	&	2.36	&	23.23	&	\rm I	\\
\rm Collinder\,350	&	2.6	&	5.3	\pm	2.68	&	4.68	\pm	0.37	&	4.11	\pm	0.43	&	0.88	\pm	0.45	&	0.78	\pm	0.4	&	7.65	&	10.28	&		\\
\rm Gulliver\,6	&	3.1	&	5.54	\pm	3.67	&	4.58	\pm	0.48	&	3.29	\pm	0.54	&	0.83	\pm	0.55	&	0.59	\pm	0.4	&	8.31	&	26.93	&		\\
\rm Gulliver\,21	&	3.7	&	5.66	\pm	5.29	&	3.47	\pm	0.57	&	2.59	\pm	0.65	&	0.61	\pm	0.58	&	0.46	\pm	0.44	&	20.12	&	34.4	&		\\
\rm Huluwa\,1$^b$	&	2.5	&	9.56	\pm	2.47	&	9.17	\pm	0.36	&	6.42	\pm	0.41	&	0.96	\pm	0.25	&	0.67	\pm	0.18	&	0.44	&	25.33	&	\rm III	\\
\rm Huluwa\,2$^b$	&	2.9	&	9.21	\pm	3.09	&	7.68	\pm	0.4	&	6.38	\pm	0.46	&	0.83	\pm	0.28	&	0.69	\pm	0.24	&	61.15	&	52.55	&		\\
\rm Huluwa\,3$^b$	&	2.6	&	7.3	\pm	2.57	&	6.51	\pm	0.36	&	5.53	\pm	0.41	&	0.89	\pm	0.32	&	0.76	\pm	0.27	&	6.58	&	73.68	&		\\
\rm Huluwa\,4$^b$	&	2.5	&	6.33	\pm	2.29	&	5.17	\pm	0.32	&	4.53	\pm	0.39	&	0.82	\pm	0.3	&	0.72	\pm	0.27	&	77.58	&	87.0	&		\\
\rm Huluwa\,5$^b$	&	2.1	&	4.55	\pm	1.72	&	3.62	\pm	0.25	&	2.35	\pm	0.31	&	0.8	\pm	0.31	&	0.52	\pm	0.21	&	10.7	&	12.33	&	\rm I	\\
\rm IC\,348	&	2.6	&	4.82	\pm	2.59	&	3.15	\pm	0.36	&	2.13	\pm	0.42	&	0.65	\pm	0.36	&	0.44	\pm	0.25	&	18.94	&	13.23	&	\rm III	\\
\rm IC\,4756	&	3.0	&	8.44	\pm	3.58	&	6.4	\pm	0.45	&	5.0	\pm	0.51	&	0.76	\pm	0.33	&	0.59	\pm	0.26	&	0.83	&	7.22	&		\\
\rm LP\,2371	&	2.8	&	6.25	\pm	3.0	&	4.08	\pm	0.42	&	2.75	\pm	0.46	&	0.65	\pm	0.32	&	0.44	\pm	0.22	&	34.35	&	76.29	&		\\
\rm LP\,2373	&	2.9	&	5.64	\pm	3.21	&	5.39	\pm	0.41	&	2.37	\pm	0.5	&	0.96	\pm	0.55	&	0.42	\pm	0.25	&	5.04	&	43.75	&	\rm I	\\
\rm LP\,2373\,gp1$^a$	&	2.5	&	6.63	\pm	2.42	&	5.52	\pm	0.34	&	5.08	\pm	0.4	&	0.83	\pm	0.31	&	0.77	\pm	0.29	&	22.18	&	42.43	&		\\
\rm LP\,2373\,gp2	&	2.5	&	8.53	\pm	2.32	&	7.3	\pm	0.33	&	6.54	\pm	0.39	&	0.86	\pm	0.24	&	0.77	\pm	0.21	&	38.6	&	74.55	&		\\
\rm LP\,2373\,gp3	&	2.5	&	5.12	\pm	2.49	&	4.51	\pm	0.36	&	4.0	\pm	0.41	&	0.88	\pm	0.43	&	0.78	\pm	0.39	&	45.31	&	72.23	&		\\
\rm LP\,2373\,gp4	&	2.5	&	6.78	\pm	2.42	&	6.37	\pm	0.33	&	6.03	\pm	0.41	&	0.94	\pm	0.34	&	0.89	\pm	0.32	&	15.69	&	35.28	&		\\
\rm LP\,2383	&	3.7	&	8.18	\pm	5.4	&	4.85	\pm	0.59	&	4.32	\pm	0.67	&	0.59	\pm	0.4	&	0.53	\pm	0.36	&	9.44	&	4.4	&	\rm II	\\
\rm LP\,2388	&	4.4	&	5.65	\pm	7.44	&	5.15	\pm	0.69	&	3.04	\pm	0.76	&	0.91	\pm	1.2	&	0.54	\pm	0.72	&	30.66	&	36.2	&	\rm I	\\
\rm LP\,2428	&	3.4	&	5.18	\pm	4.54	&	4.34	\pm	0.52	&	3.28	\pm	0.6	&	0.84	\pm	0.74	&	0.63	\pm	0.57	&	16.17	&	55.57	&	\rm III	\\
\rm LP\,2429	&	3.5	&	8.67	\pm	4.84	&	4.63	\pm	0.54	&	2.51	\pm	0.64	&	0.53	\pm	0.3	&	0.29	\pm	0.18	&	13.24	&	40.47	&	\rm III	\\
\rm LP\,2439	&	2.2	&	5.16	\pm	1.86	&	4.57	\pm	0.28	&	4.05	\pm	0.33	&	0.89	\pm	0.32	&	0.78	\pm	0.29	&	48.83	&	52.34	&		\\
\rm LP\,2441	&	2.1	&	6.57	\pm	1.63	&	5.35	\pm	0.25	&	4.65	\pm	0.31	&	0.81	\pm	0.21	&	0.71	\pm	0.18	&	28.15	&	66.49	&		\\
\rm LP\,2442	&	1.4	&	6.93	\pm	0.64	&	6.07	\pm	0.11	&	3.96	\pm	0.15	&	0.88	\pm	0.08	&	0.57	\pm	0.06	&	9.57	&	38.62	&	\rm I	\\
\rm LP\,2442\,gp1$^a$	&	0.7	&	5.34	\pm	0.12	&	4.48	\pm	0.06	&	2.92	\pm	0.05	&	0.84	\pm	0.02	&	0.55	\pm	0.02	&	38.23	&	69.89	&	\rm I	\\
\rm LP\,2442\,gp2$^a$	&	0.8	&	6.87	\pm	0.19	&	5.15	\pm	0.06	&	3.56	\pm	0.06	&	0.75	\pm	0.02	&	0.52	\pm	0.02	&	59.94	&	83.21	&	\rm III	\\
\rm LP\,2442\,gp3$^a$	&	0.8	&	5.55	\pm	0.16	&	2.86	\pm	0.06	&	2.6	\pm	0.06	&	0.52	\pm	0.02	&	0.47	\pm	0.02	&	12.2	&	37.34	&	\rm II	\\
\rm LP\,2442\,gp4$^a$	&	1.2	&	5.38	\pm	0.44	&	4.91	\pm	0.08	&	2.42	\pm	0.1	&	0.91	\pm	0.08	&	0.45	\pm	0.04	&	58.54	&	42.31	&	\rm I	\\
\rm LP\,2442\,gp5$^a$	&	0.8	&	8.64	\pm	0.17	&	4.12	\pm	0.07	&	1.69	\pm	0.06	&	0.48	\pm	0.01	&	0.2	\pm	0.01	&	71.93	&	50.65	&	\rm III	\\
\rm Mamajek\,4	&	3.0	&	7.07	\pm	3.45	&	5.98	\pm	0.46	&	5.63	\pm	0.52	&	0.85	\pm	0.42	&	0.8	\pm	0.4	&	34.1	&	82.81	&		\\
\rm NGC\,1901	&	2.3	&	5.0	\pm	1.96	&	4.44	\pm	0.29	&	3.25	\pm	0.35	&	0.89	\pm	0.35	&	0.65	\pm	0.26	&	10.1	&	59.03	&	\rm III	\\
\rm NGC\,1977	&	2.4	&	4.97	\pm	2.24	&	3.83	\pm	0.3	&	2.46	\pm	0.38	&	0.77	\pm	0.35	&	0.49	\pm	0.24	&	37.3	&	87.23	&		\\
\rm NGC\,1980	&	2.7	&	10.52	\pm	2.66	&	7.97	\pm	0.37	&	3.67	\pm	0.42	&	0.76	\pm	0.19	&	0.35	\pm	0.1	&	14.61	&	58.85	&	\rm III	\\
\rm NGC\,2451B	&	2.7	&	6.0	\pm	2.89	&	5.36	\pm	0.38	&	4.37	\pm	0.46	&	0.89	\pm	0.43	&	0.73	\pm	0.36	&	5.89	&	38.24	&		\\
\rm NGC\,3228	&	2.9	&	4.36	\pm	3.25	&	3.0	\pm	0.41	&	2.34	\pm	0.48	&	0.69	\pm	0.52	&	0.54	\pm	0.41	&	0.32	&	24.11	&		\\
\rm NGC\,3532	&	3.4	&	12.32	\pm	4.52	&	9.7	\pm	0.53	&	5.06	\pm	0.6	&	0.79	\pm	0.29	&	0.41	\pm	0.16	&	1.21	&	11.37	&	\rm III	\\
\rm NGC\,6405	&	4.4	&	9.87	\pm	7.42	&	4.6	\pm	0.69	&	3.26	\pm	0.77	&	0.47	\pm	0.36	&	0.33	\pm	0.26	&	3.82	&	12.03	&		\\
\rm NGC\,6475	&	2.0	&	9.8	\pm	1.52	&	8.0	\pm	0.23	&	4.73	\pm	0.29	&	0.82	\pm	0.13	&	0.48	\pm	0.08	&	2.05	&	5.49	&	\rm I	\\
\rm NGC\,7058	&	2.7	&	4.45	\pm	2.81	&	3.24	\pm	0.38	&	2.43	\pm	0.45	&	0.73	\pm	0.47	&	0.55	\pm	0.36	&	19.24	&	72.08	&		\\
\rm NGC\,7092	&	2.3	&	6.37	\pm	2.01	&	5.11	\pm	0.3	&	4.01	\pm	0.35	&	0.8	\pm	0.26	&	0.63	\pm	0.21	&	5.5	&	82.13	&		\\
\rm Pleiades$^b$	&	0.9	&	7.9	\pm	0.23	&	7.06	\pm	0.07	&	4.02	\pm	0.07	&	0.89	\pm	0.03	&	0.51	\pm	0.02	&	17.79	&	10.35	&	\rm I	\\
\rm Praesepe	&	1.6	&	7.37	\pm	0.97	&	5.32	\pm	0.15	&	4.95	\pm	0.2	&	0.72	\pm	0.1	&	0.67	\pm	0.09	&	11.14	&	43.6	&		\\
\rm Roslund\,5	&	4.1	&	5.67	\pm	6.39	&	4.51	\pm	0.64	&	4.24	\pm	0.71	&	0.8	\pm	0.9	&	0.75	\pm	0.85	&	9.21	&	33.44	&		\\
\rm RSG\,7	&	2.4	&	4.74	\pm	2.27	&	3.8	\pm	0.34	&	2.36	\pm	0.4	&	0.8	\pm	0.39	&	0.5	\pm	0.25	&	9.39	&	33.79	&	\rm I	\\
\rm RSG\,8	&	4.8	&	8.6	\pm	8.99	&	7.01	\pm	0.76	&	6.1	\pm	0.85	&	0.82	\pm	0.86	&	0.71	\pm	0.75	&	20.71	&	44.6	&		\\
\rm Stephenson\,1	&	2.6	&	5.72	\pm	2.57	&	5.23	\pm	0.36	&	4.42	\pm	0.41	&	0.91	\pm	0.42	&	0.77	\pm	0.35	&	26.02	&	53.14	&		\\
\rm Stock\,1	&	2.4	&	5.41	\pm	2.23	&	4.83	\pm	0.33	&	3.16	\pm	0.39	&	0.89	\pm	0.37	&	0.58	\pm	0.25	&	2.66	&	81.57	&	\rm I	\\
\rm Stock\,12	&	2.7	&	6.5	\pm	2.73	&	4.62	\pm	0.38	&	2.51	\pm	0.44	&	0.71	\pm	0.3	&	0.39	\pm	0.18	&	10.3	&	88.02	&	\rm III	\\
\rm Stock\,23	&	4.0	&	7.52	\pm	6.15	&	3.83	\pm	0.65	&	2.78	\pm	0.71	&	0.51	\pm	0.43	&	0.37	\pm	0.32	&	33.59	&	57.15	&		\\
\rm UBC\,7$^b$	&	2.0	&	6.95	\pm	1.59	&	4.66	\pm	0.26	&	3.83	\pm	0.28	&	0.67	\pm	0.16	&	0.55	\pm	0.13	&	12.48	&	26.29	&		\\
\rm UBC\,19	&	3.5	&	3.94	\pm	4.87	&	3.4	\pm	0.56	&	2.23	\pm	0.62	&	0.86	\pm	1.07	&	0.57	\pm	0.72	&	14.83	&	34.2	&	\rm I	\\
\rm UBC\,31	&	3.2	&	6.31	\pm	4.06	&	5.74	\pm	0.5	&	4.67	\pm	0.57	&	0.91	\pm	0.59	&	0.74	\pm	0.48	&	6.78	&	33.83	&		\\
\rm UBC\,31\,gp1$^a$	&	3.4	&	6.07	\pm	4.56	&	4.13	\pm	0.53	&	3.07	\pm	0.61	&	0.68	\pm	0.52	&	0.51	\pm	0.39	&	1.68	&	11.99	&		\\
\rm UBC\,31\,gp2$^a$	&	3.0	&	6.99	\pm	3.6	&	6.1	\pm	0.46	&	4.6	\pm	0.53	&	0.87	\pm	0.45	&	0.66	\pm	0.35	&	6.1	&	27.11	&	\rm III	\\
\rm UPK\,82	&	3.7	&	4.58	\pm	5.24	&	3.49	\pm	0.57	&	2.65	\pm	0.66	&	0.76	\pm	0.88	&	0.58	\pm	0.68	&	32.52	&	72.08	&		\\
